Dependently Typed Knowledge Graphs

Reasoning over knowledge graphs is traditionally built upon a hierarchy of languages in the Semantic Web Stack. Starting from the Resource Description Framework (RDF) for knowledge graphs, more advanced constructs have been introduced through various syntax extensions to add reasoning capabilities to knowledge graphs. In this paper, we show how standardized semantic web technologies (RDF and its query language SPARQL) can be reproduced in a unified manner with dependent type theory. In addition to providing the basic functionalities of knowledge graphs, dependent types add expressiveness in encoding both entities and queries, explainability in answers to queries through witnesses, and compositionality and automation in the construction of witnesses. Using the Coq proof assistant, we demonstrate how to build and query dependently typed knowledge graphs as a proof of concept for future works in this direction.

==> defManSSR.tex <==
%=======================================================================
% A listing mode for ssr Gallina (Assia Mahboubi 2007)

\lstdefinelanguage{SSR} {

% Anything between $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Infix, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex,
Implicits, Types,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Admitted, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections,
inside, outside, Locate, Eval,
About, Check},


% Gallina
morekeywords=[2]{forall, exists2, fun, fix, cofix, struct, 
      match, with, end, as, in, return, let, if, of, is, isn't, then, else,
      for, nosimpl, where,
      witness_sb, witness_mb, witness_gc, witness_cw, witness_mm,
      },
% 'of' is removed from this list as it occurs in comments.

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{
         pose, set, move, case, elim, apply, clear, exists,
            hnf, intro, intros, generalize, rename, pattern, after,
            destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
         gen, generally, abstract,
            assert, cut, trivial, revert, bool_congr, nat_congr, vm_compute,
         symmetry, transitivity, auto, split, left, right,
         autorewrite, lia, intlia},

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate, admit},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=
%       {->}{{$\rightarrow\ $}}2
%       {->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2
%       {<-}{{\tt <-}}2
%       {>->}{{$\mapsto$}}3
%       {<}{{$<\;\;$}}1
%       {<=}{{$\leq\;\;$}}1
%       {>=}{{$\geq\;\;$}}1
%       {<>}{{$\neq$}}1
%        {/\\}{{$\wedge\;\;$}}2
%        {\\/}{{$\vee\;\;$}}2
%       {^~}{{\textvisiblespace$\;\;$}}2
%       {~~}{{$\lnot\;\;$}}2
%       {<->}{{$\leftrightarrow\;$}}3
%       {<=>}{{$\Leftrightarrow\;$}}3
%       {:nat}{{$~\in\mathbb{N}$}}3
%	{fforall\ }{{$\forall_f\,$}}1
	{forall\ }{{$\forall\ \!$}}1
%	{exists\ }{{$\exists\ \!$}}1
%       {MAPLE}{{\raisebox{-0.8cm}[0cm][0cm]{\hspace{18mm}\includegraphics[width=1cm]{maple}}}}1
%	{^2}{{$^2$}}1
	{^3}{{$^3$}}1
	{^4}{{$^4$}}1
	{^5}{{$^5$}}1
	{^6}{{$^6$}}1
%       {negb}{{$\neg$}}1
%       {spp}{{:*:\,}}1
%       {~}{{$\sim$}}1
%       {\\in}{{$\in\;$}}1
%       {/\\}{$\land\,$}1
%       {:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
%       {=>}{{\tt =>}}2
%       {:=}{{{\tt:=}\,\,}}2
%       {==}{{$\equiv$}\,}2
%       {!=}{{$\neq$}\ }2
%       {_cf0}{{$_{{0}}$}}1
%       {_cf1}{{$_{{1}}$}}1
%       {_cf2}{{$_{{2}}$}}1
%       {_cf0_0}{{$_{{00}}$}}1
%       {^-1}{{$^{-1}$}}1
%       {elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2
,

% Comments delimiters, we do turn this off for the manual
%comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
%basicstyle=\ttfamily\footnotesize,
basicstyle=\ttfamily\small,
% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,

% do not eat spaces after) in inline
keepspaces=true,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{dkviolet}},

% Style for Gallina keywords
keywordstyle=[2]{\ttfamily\color{dkgreen}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
%commentstyle=\rmfamily,

}
